MiM: Mask in Mask Self-Supervised Pre-Training for 3D Medical Image Analysis

The Vision Transformer (ViT) has demonstrated remarkable performance in Self-Supervised Learning (SSL) for 3D medical image analysis. Masked AutoEncoder (MAE) for feature pre-training can further unleash the potential of ViT on various medical vision tasks. However, due to large spatial sizes with much higher dimensions of 3D medical images, the lack of hierarchical design for MAE may hinder the performance of downstream tasks. In this paper, we propose a novel \textit{Mask in Mask (MiM)} pre-training framework for 3D medical images, which aims to advance MAE by learning discriminative representation from hierarchical visual tokens across varying scales. We introduce multiple levels of granularity for masked inputs from the volume, which are then reconstructed simultaneously ranging at both fine and coarse levels. Additionally, a cross-level alignment mechanism is applied to adjacent level volumes to enforce anatomical similarity hierarchically. Furthermore, we adopt a hybrid backbone to enhance the hierarchical representation learning efficiently during the pre-training. MiM was pre-trained on a large scale of available 3D volumetric images, \textit{i.e.,} Computed Tomography (CT) images containing various body parts. Extensive experiments on thirteen public datasets demonstrate the superiority of MiM over other SSL methods in organ/lesion/tumor segmentation and disease classification. We further scale up the MiM to large pre-training datasets with more than 10k volumes, showing that large-scale pre-training can further enhance the performance of downstream tasks. The improvement also concluded that the research community should pay more attention to the scale of the pre-training dataset towards the healthcare foundation model for 3D medical images.

==> algorithms/pipeline.tex <==
% \IncMargin{0.5em}
\begin{algorithm}[ht] \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up} \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress} \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\small
 	\caption{MiM: \textbf{M}ask in \textbf{M}ask Self-Supervised Pre-training framework}\label{alg:overall}
	\Input{}
    {$\mathcal{D}$, $\tau$  \qquad\qquad dataset and the transformations;}\\
    {$\theta$, $s_{\theta}$ \qquad\space initial parameters for encoder, encoder;}\\
    {$\xi$, $d_{\xi}$       \qquad\space initial parameters for decoder, decoder;}\\
    {$\iota$, $\mathcal{H}$ \qquad\space initial parameters for aggregation and projector heads;}\\
    {$\operatorname{optimizer}$ \qquad\space  optimizer, updated parameters via gradient backwards;}\\
    {$K$, $B$, $\mu$ \qquad\space  pre-training steps, batch size and learning rate;}
	 \BlankLine
	 \For{$k\leftarrow 1$ \KwTo $K$}{
		\tcp{sample one batches from dataset}
        $\mathcal{B}$ $\leftarrow$ $\left\{\left\{x\right\} \sim \mathcal{D}\right\}_{i=1}^B $
	 	\For{i, $x\in \mathcal{B}$}{

		% \tcp{sample image transformations for three-level volumes}
        % $\tau, t^m_1$, $t^m_2$, $t^m_3$ $\sim$ $\mathcal{T}$;
		% $x^1\leftarrow \tau(x)$;
		% \hfill \tcp{crop to sub-volume}
        % $\tilde{V_1}, V_1\leftarrow t^m_1(x_1)$ and $X_2\leftarrow \tilde{V_1}$;
		% \hfill \tcp{visible and invisible tokens for level 1}
        % $\tilde{V_2}, V_2\leftarrow t^m_2(x_2)$, $x_2\in X_2$ and $X_3\leftarrow \tilde{V_2}$;
		% \hfill \tcp{visible and invisible tokens for level 2}
        % $\tilde{V_3}, V_3\leftarrow t^m_3(x_3)$; $x_3\in X_3$
		% \hfill \tcp{visible and invisible tokens for level 3}
		Apply multi-level masked volume generation for $x$ to obtain $x^1$, $x^2$ and $x^3$;\\
		Apply Eq.(2) for $x^1$ to obtain $\mathcal{L}_R^1$ with $s_\theta$ and $d_\xi$;\\
		Apply Eq.(2) for $x^2$ to obtain $\mathcal{L}_R^2$ with $s_\theta$ and $d_\xi$;\\
		Apply Eq.(2) for $x^3$ to obtain $\mathcal{L}_R^3$ with $s_\theta$ and $d_\xi$;\\
		Apply Eq.(3) to obtain $\mathcal{L}^R$ with $s_\theta$ and $d_\xi$;\\
		Apply Eq.(6) for $x^2$ and $x^1$ to obtain $\mathcal{L}_C^{1,2}$ with $s_\theta$ and $\mathcal{H}_\iota$;\\
		Apply Eq.(6) for $x^3$ and $x^2$ to obtain $\mathcal{L}_C^{2,3}$ with $s_\theta$ and $\mathcal{H}_\iota$;\\
		Apply Eq.(7) to obtain $\mathcal{L}^C$ with $s_\theta$ and $\mathcal{H}_\iota$;\\
		% \hfill \tcp{compute level 2 reconstruction loss}
		% Apply Eq.(3) for $V_3$ to obtain $\mathcal{L}^R_3$ with $s_\theta$ and $d_\xi$;
		% \hfill \tcp{compute level 3 reconstruction loss}
		% Apply Eq.(4) for level 1 $V_1$ and level 2 $V_2$ representation to obtain $\mathcal{L}^C_{12};$ with $s_\theta$, $d_\xi$ and $\mathcal{H}_\iota$.
		% \hfill \tcp{calculate cross-alignment loss for level 1 and level 2}
		% Apply Eq.(4) for level 2 $V_2$ and level 3 $V_3$ representation to obtain $\mathcal{L}^C_{23};$ with $s_\theta$, $d_\xi$ and $\mathcal{H}_\iota$.
		% \hfill \tcp{calculate cross-alignment loss for level 2 and level 3}
		Apply Eq.(10) to obtain the final loss $\mathcal{L}$
		}
        $\delta \theta \leftarrow \frac{1}{B} \sum_{i=1}^B\left(\partial_\theta \mathcal{L} \right) ;$
		% \hfill \tcp{compute the loss gradient w.r.t $\theta$}
		$\delta \xi \leftarrow \frac{1}{B} \sum_{i=1}^B\left(\partial_\xi \mathcal{L} \right) ;$\\
		$\delta \iota \leftarrow \frac{1}{B} \sum_{i=1}^B\left(\partial_\iota \mathcal{L} \right) ;$\\
        $\theta \leftarrow \operatorname{optimizer}(\theta, \delta_\theta, \mu) ;$
		% \hfill \tcp{update parameters of the network}
        $\xi \leftarrow \operatorname{optimizer}(\xi, \delta_\xi, \mu) ;$ \\
        $\iota \leftarrow \operatorname{optimizer}(\iota, \delta_\iota, \mu) ;$ \\
 	 }
    %$\delta \theta \leftarrow \frac{1}{N} \sum_{i=1}^N\left(\partial_\theta l_{\theta, \xi}^{G V S L, i}+l_{\theta, i}^{M S E, i}\right) ; \\ & \delta \xi \leftarrow \frac{1}{N} \sum_{i=1}^N \partial_{\xi} l_{\theta, \xi}^{G V S L, i} ; \\ & \delta \iota \leftarrow \frac{1}{N} \sum_{i=1}^N \partial_\iota l_{\theta, i}^{M S E, i} ; \\ & \theta \leftarrow \operatorname{optimizer}(\theta, \delta \theta, \eta) ; \\ & \xi \leftarrow \operatorname{optimizer}(\xi, \delta \xi, \eta) ; \\ & \iota \leftarrow \operatorname{optimizer}(\iota, \delta \iota, \eta)$
	\Output{$s_{\theta}$ \hfill \tcp{the pre-trained backbone encoder}}
 	 \end{algorithm}
% \DecMargin{0.5em}
